Performance Analysis of UNet and Variants for Medical Image Segmentation

Medical imaging plays a crucial role in modern healthcare by providing non-invasive visualisation of internal structures and abnormalities, enabling early disease detection, accurate diagnosis, and treatment planning. This study aims to explore the application of deep learning models, particularly focusing on the UNet architecture and its variants, in medical image segmentation. We seek to evaluate the performance of these models across various challenging medical image segmentation tasks, addressing issues such as image normalization, resizing, architecture choices, loss function design, and hyperparameter tuning. The findings reveal that the standard UNet, when extended with a deep network layer, is a proficient medical image segmentation model, while the Res-UNet and Attention Res-UNet architectures demonstrate smoother convergence and superior performance, particularly when handling fine image details. The study also addresses the challenge of high class imbalance through careful preprocessing and loss function definitions. We anticipate that the results of this study will provide useful insights for researchers seeking to apply these models to new medical imaging problems and offer guidance and best practices for their implementation.

==> sections/Acknowledgements.tex <==
\chapter*{Acknowledgements}
% This page is where you have the opportunity to give thanks to anyone, or anything that inspired or helped you with your project.



% \vspace{3cm}

% \begin{tikzpicture}[
%     node distance = 0mm and 1mm,
% box/.style = {text width=15cm, font=\normalsize},  % define nodes style
%                     ]
% \node (n1) [box,draw] {I certify that the work presented in the dissertation is my own unless referenced.\\
% \vspace{1cm}
% %replace the image signature_example with your own image of your signature
% Signature: \includegraphics[width=0.2\textwidth]{images/signature_example.png}\\ 
% \vspace{1cm}
% Date:
% \vspace{1cm}
% };
% \end{tikzpicture}


% \vspace{1cm}
% Total words:  


Firstly, I want to convey my deep appreciation to my family for their unwavering support. I would also like to extend my thanks to my esteemed educators, with a special mention to Prof. George Ghinea, Elena Boguslavskaya, Dr. Alessandro Pandini, and my supervisor, Dr. Yongmin Li, for their invaluable guidance.\\\\



\begin{tcolorbox}[mybox]
\begin{minipage}{0.8\textwidth}
    I certify that the work presented in the dissertation is my own unless referenced.\\\\
    Signature \\\\
    \includegraphics[width=3cm]{images/signature.png}\\
\today
\end{minipage}
\end{tcolorbox}
\textbf{\\TOTAL NUMBER OF WORDS: 13997}

\newpage








==> titlepage.tex <==
\begin{titlepage}
    \begin{center}
        \vspace*{0.1cm}
        
          
        \includegraphics[width=0.6\textwidth]{images/brunel-logo.jpg}
        
        \large
         \textbf{Department of Computer Science}
         \vspace{1cm}
         
         \textbf{MSc in Artificial Intelligence}
         \vspace{1cm}
         
         Academic Year 2022-2023
         
         
         \vspace{2cm}
        
        
        \LARGE
        \textbf{Medical Image Segmentation: Illuminating Anatomy with UNet and Variants}
        
        
        \vspace{1.5cm}
        \large
        \textbf{Walidul Alam Ehab}
        
        2257956
        
       % \vfill
        \vspace{1.5cm}
        A report submitted in partial fulfilment of the requirement for the degree of Master of Science

        
        \vspace{0.8cm}
      \begin{flushright}
        \footnotesize
        Brunel University London \\
        Department of Computer Science\\
        Uxbridge\\
        Middlesex\\
        UB8 3PH\\
        United Kingdom \\
        T: +44 1895 203397\\
        F: +44 (0) 1895 251686\\
        \end{flushright}
        
    \end{center}
\end{titlepage}
